A framework for deadlock detection in core ABS

We present a framework for statically detecting deadlocks in a concurrent object-oriented language with asynchronous method calls and cooperative scheduling of method activations. Since this language features recursion and dynamic resource creation, deadlock detection is extremely complex and state-of-the-art solutions either give imprecise answers or do not scale. In order to augment precision and scalability we propose a modular framework that allows several techniques to be combined. The basic component of the framework is a front-end inference algorithm that extracts abstract behavioural descriptions of methods, called contracts, which retain resource dependency information. This component is integrated with a number of possible different back-ends that analyse contracts and derive deadlock information. As a proof-of-concept, we discuss two such back-ends: (i) an evaluator that computes a fixpoint semantics and (ii) an evaluator using abstract model checking.

==> case-study.tex <==

% Presentation of the case study with introduction of the basic principles of ABS-core:
% \begin{itemize}
% \item object oriented language
% \item cogs, synchronous/asynchronous calls, futures, awaits/gets
% \item other things?
% \end{itemize}
% 
% And presents where (or why) there are risks of deadlocks.



{The Fredhopper Access Server (FAS) is a distributed
concurrent object-oriented system that provides search and merchandising services to eCommerce companies.
%Briefly, FAS provides to its clients structured search capabilities within the
%client's data. 
%Each FAS installation is deployed to a customer according to the
%FAS deployment architecture (See Fig~\ref{casestudy}).
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=10cm]{src/deploymentmodels}
%\caption{\label{casestudy} An example FAS deployment}
%\vspace{-0.5cm}
%\end{figure}
%
% \begin{figure}[t]
% \centering
% \includegraphics[width=12.2cm]{sequence}
% \caption{\label{interaction} Replication interaction}
% \vspace{-0.5cm}
% \end{figure}
%
FAS consists of a set of live environments and a single staging environment. A live
environment processes queries from client web applications via web services and
aims to provide a constant query capacity to client-side web applications.
%
A staging environment is responsible for receiving data updates,
and distributing the resulting indices across all live
environments according to the \emph{Replication Protocol}.
%
The \emph{Replication Protocol} %is implemented by the
%\emph{Replication System} that 
has a single \emph{SyncServer} module 
%at the staging environment 
and one \emph{SyncClient} module for each live environment.
In turn, the \emph{SyncServer} determines the schedule of replications, as well
as their content, while a \emph{SyncClient} receives data and configuration
updates according to the schedule.\looseness-1 \par}

% \begin{figure}[b!]
% \centering
% \includegraphics[width=10cm]{casestudyseq}
% \caption{\label{casestudyseq} Interaction between SyncClient, ConnectionThread, Snapshot 
% and Coordinator in a replication session.}
% \vspace{-0.5cm}
% \end{figure}

%\subsection{Replication Protocol}
{The \emph{SyncServer} communicates to \emph{SyncClient}s by creating
\emph{Worker} objects, which serve as the interface to the server-side of the
\emph{Replication Protocol}.
%
On the other hand, \emph{SyncClient}s schedule and create \emph{ClientJob} objects to
handle communications to the client-side of the \emph{Replication Protocol}.
%
When transferring data between the staging and the live environments, it is
critical that the data remains \emph{immutable}. To enforce immutability, without
interfering with read/write accesses to the staging environment's underlying
file system, the \emph{SyncServer} creates a \emph{Snapshot} object that encapsulates a
snapshot of the necessary part of the staging environment's file system, and
periodically \emph{refreshes} it against the file system. This guarantees
immutability of data until their update is deemed safe.
The \emph{SyncServer} uses a \emph{Coordinator} object to determine the safe state in which the
\emph{Snapshot} can be refreshed.\looseness-1 \par}
%
% \Cref{interaction} shows a UML sequence diagram concerning parts of the
% replication protocol with the interaction between a SyncClient, a ClientJob, a
% Worker, a SyncServer, a Coordinator and a Snapshot.
% The figure assumes that SyncClient has already established connection with a SyncServer and 
% shows how a ClientJob from the SyncClient and a Worker from a SyncServer are 
% instantiated for interaction. For the purpose of this paper
% we consider this part of the Replication Protocol as a \emph{replication session}.

\ifIFM
\else
\paragraph{Modeling The Replication Protocol.}
%
Figure~\ref{inf} shows some data types and interfaces used to model the
\emph{Replication Protocol}. 
%The interface \Abs{ClientJob} models a ClientJob, while
%interface \Abs{DataBase} models the database of the underlying file system of
%the SyncClient.
%
The algebraic data type (ADT) \Abs{Content} models the file system of
the environments. % in \ABS. 
ADTs permit to specify
immutable values %in functional expressions 
and to abstract away from
implementation details such as hardware environment, file content, or
operating system specifics.
% 
More in detail, \Abs{Content} is either a \Abs{File},
where an integer (e.g., its size) is taken to represent the content of a single
file, or it is a directory \Abs{Dir}, with a mapping of names to \Abs{Content},
thereby modeling a file system structure with hierarchical name space.  

\begin{figure*}[t]
\begin{absexamplen}
data Content = File(Int content) | Dir(Map<String,Content>);

interface ClientJob {
  Bool register(Int sid);
  Maybe<Int> file(String id);
}

interface DataBase {
  Bool hasFile(String id);
  Content getContent(String id);
}
\end{absexamplen}
\caption{\label{inf} Data types and Interfaces}
\end{figure*}

The interface \Abs{ClientJob} has two methods: \Abs{register} and
\Abs{file}. The former method  takes
an integer parameter \Abs{sid} that identifies the version of the data the
replication would update the live environment to. It tests whether the
live environment already contains this update (it also prepares the
underlying database for a possible new incoming update, but this is
irrelevant for our presentation).  The method \Abs{file} takes a
\Abs{String} value specifying the absolute path to a file stored in
the live environment and returns a \Abs{Maybe} value which is either
an integer representing the file content or the value \Abs{Nothing} if
no such file exists.

The interface \Abs{Database} has also two methods, both taking in input
a path to a file. The method \Abs{hasFile}
%takes the
%absolute path to a file and 
tests the presence in the live
environment of the file addressed by the path in input. The method \Abs{getContent}
returns a \Abs{Content} value representing the content of the file
identified by the path in input.
%
Figure~\ref{filem} shows the implementation of \Abs{file} in the
class \Abs{ClientJobImpl}. This class has an instance field \Abs{db} of type
\Abs{DataBase}. The ADT function
\Abs{isFile} takes a \Abs{Content} value and returns \Abs{True} whenever
the input  records a file; \Abs{content} is a partial
\emph{selector} function that returns the argument of the constructor
\Abs{File}.

\begin{figure*}[t]
\begin{absexamplen}
def Bool isFile(Content c) = case { File(_) => True; _ => False; };

class ClientJobImpl(Database db) implements ClientJob {
  Maybe<Int> file(String id) {
    Fut<Bool> he = db!hasFile(id); await he?; 
    Bool hasfile = he.get; 
    Maybe<Int> result = Nothing;
    if (hasfile) {
      Fut<Content> f = db!getContent(id); await f?; Content c = f.get;
      if (isFile(c)) {
        result = Just(content(c));
      }
    }
    return result; 
  }
}
\end{absexamplen}
\caption{\label{filem}Method \Abs{file} and auxiliary function}
\end{figure*}

The method \Abs{file} is implemented using key features of {\coreABS}:
asynchronous invocations, message passing, active waiting, and future types.
In particular, \Abs{file} first calls asynchronously \Abs{hasFile(id)} on  
\Abs{db}  to
access the underlying file system. This invocation spawns a new task and
returns a \emph{future} variable \Abs{he} as a place-holder for the
result of the call to \Abs{hasFile(id)}. The statement \Abs{await he?}
suspends the current task until \Abs{he} is resolved. The result, once available,
can be accessed with \Abs{he.get}.
\fi

\ifIFM
\else
\paragraph{Deadlock freedom.}
As the \emph{Replication Protocol} is a program with multiple
threads interacting concurrently, there are risks of deadlocks.
%
\iffalse
\begin{figure*}[t]
\begin{center}
\includegraphics[width=8cm]{src/sequence}
\end{center}
\caption{UML sequence diagram of a replication job}
\label{fig:rep1}
\end{figure*}
%
Figure \ref{fig:rep1} shows how for each scheduled replication session, a
\Abs{ClientJob} object is created to interact with the staging environment via a
\Abs{Worker} object. 
\fi
The informal description of the
interaction follows.

\begin{sloppypar}
\begin{quote}
For each scheduled replication session, the SyncClient creates a ClientJob.
This ClientJob first connects to a Worker
(\Abs{Acceptor.getConnection}); this connection creates a new \Abs{Worker} object. 
The ClientJob then acquires from the
ConnectionThread the next schedule for this replication session
(\Abs{ClientJob.getSchedules()}) and notifies the SyncClient
(\Abs{SyncClient.schedule()}). The SyncClient \emph{waits} for the termination
of the current
ClientJob before proceeding with the next scheduled replication
session. In the meantime the current ClientJob receives replication updates from
the Worker \Abs{ClientJob.sendItems()}.
\end{quote} 
\end{sloppypar}
\fi





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "subm-SoSyM"
%%% End: 

